Everyday AR through AI-in-the-Loop

This workshop brings together experts and practitioners from augmented reality (AR) and artificial intelligence (AI) to shape the future of AI-in-the-loop everyday AR experiences. With recent advancements in both AR hardware and AI capabilities, we envision that everyday AR -- always-available and seamlessly integrated into users' daily environments -- is becoming increasingly feasible. This workshop will explore how AI can drive such everyday AR experiences. We discuss a range of topics, including adaptive and context-aware AR, generative AR content creation, always-on AI assistants, AI-driven accessible design, and real-world-oriented AI agents. Our goal is to identify the opportunities and challenges in AI-enabled AR, focusing on creating novel AR experiences that seamlessly blend the digital and physical worlds. Through the workshop, we aim to foster collaboration, inspire future research, and build a community to advance the research field of AI-enhanced AR.

==> trash.tex <==
\section{Introduction}

% The advent of generative AI, large language models, and new foundation models in computer vision have fostered numerous technological innovations in AI research and its applications. However, interface design and interaction with AI technologies is predominantly confined to graphical user interfaces (GUIs) on computers or smartphones. 
% We believe that the next step in Human-AI Interaction should be oriented towards "real-world" AI interfaces, where the AI technology naturally and seamlessly integrates into our everyday life by blending bits and atoms. By blending AI with extended reality (XR), we can enable human-AI interactions that are more physical, spatial, and context-aware, beyond the limitations of current GUI-based interfaces.
% However, despite immense potential, the integration of XR and AI has barely been investigated yet.% not fully investigated yet. 
% We believe it is a critical future direction in HCI research and there is need to build, connect, and grow a community around these shared domains to collectively push the boundary of AI-XR research. %It is important for HCI researchers to the future direction of XR and AI research. And more importantly, it is important to build, connect, and grow the research community to collectively push the boundary of XR and AI research.




% The goal of this XR and AI workshop (\url{https://xr-and-ai.github.io}) is to bring XR and AI researchers together to gather insights, facilitate collaboration, and shape the future of real-world-oriented human-AI interaction research.
% In particular, we aim to develop a strategic roadmap for future directions, which will, for instance, define key research questions, explore new application domains, and identify the challenges and opportunities in AI-XR research.
% But foremost, this workshop will bring together a research community that will collaborate on this focus in the future. 
% Finally, we plan to establish the groundwork for a reference paper to inform future research and to initiate a proposal for follow-up activities, like workshops and seminars, to continue growing the momentum towards these research efforts.





% \subsubsection*{\textbf{Explainability (XAI) in XR}}


% \subsubsection*{\textbf{Prototyping XR with AI}}
% As XR interfaces become more accessible to end users, lowering the barrier to design and develop XR applications becomes increasingly critical~\cite{nebeling2022xr}. Current tools primarily focus on developing applications and experiences for static contexts. Therefore, a major challenge lies in enabling non-technical users to author adaptive behaviors~\cite{du2023rapsai}. This is particularly crucial in the development of tangible interfaces, which could unlock significant potential for immersive XR experiences~\cite{monteiro2023teachable, suzuki2020realitysketch}.


% \subsubsection*{\textbf{LLMs for XR}}
% LLMs for XR focus specifically on the exploration of large language models to augment mixed reality experiences.
% Languages are an important part of XR experiences, including in-person communication~\cite{liao2022realitytalk, liu2023visual}, physical document reading~\cite{li2019holodoc}, and language learning.
% How can we leverage the LLMs to naturally augment such interactions, instead of explicitly typing questions on the screen? 
% Beyond text-based interaction, what kind of new applications are possible by integrating the recent advances in multi-modal LLMs to XR environment? 

% \subsubsection*{\textbf{Adaptive and Context-Aware XR}}
% Adaptive and context-aware XR focuses on the development of XR interfaces that seamlessly blend into the user's everyday environment~\cite{lindlbauer2019context, grubert2017pervasive}. Current research investigates how computational methods from optimization and machine learning can be leveraged to create XR interfaces that understand and adapt to the context of users and their environment. 
% %How may incorporating adaptivity into existing XR applications areas benefit users and enable novel functionality?
% %What new applications may be enabled with advances in adaptive XR? 
% %The goal is to create interfaces that can be deployed in uncontrolled environments, adapting to varying contexts and user states. 

% \subsubsection*{\textbf{Generative XR}}
% We explore the integration of generative AI for XR applications.
% For instance, by leveraging the recent advances in image generation such as GAN and Stable Diffusion, there is a vast potential to transform various aspects of XR interactions, such as content creation~\cite{liu20223dall} 3D and avatar animation \cite{ahuja2021coolmoves}, and immersive environment design \cite{gal2014flare}.
% Generative XR is not limited to image generation, but can be integrated with generative AI for text, motion, video, and 3D object as well. 
% In particular, we are interested in understanding how generative AI can leverage the unique physical and spatial aspects of XR applications, such as 3D scene understanding and spatial and tangible interactions. What are the challenges and possibilities in such integration?

% \subsubsection*{\textbf{Explainable AI for XR}}
% Explainable AI for XR addresses the growing need for user-friendly interfaces that help users understand, customize, and interact with mixed reality applications~\cite{xu2023xair}. It involves creating prototyping tools aimed at making XR experiences more accessible and understandable. The challenge is how to enable non-technical users to author adaptive behaviors and how conventional interface prototyping methods can be adapted for the development of adaptive XR.

% \subsubsection*{\textbf{Other XR x AI Topics}}
% We also welcome any possible XR and AI themes, such as intelligent interaction techniques, AI-enabled accessibility in XR, new evaluation methodologies, and real-world-oriented human-AI interaction.




% \vspace{0.2cm}\noindent
% \textbf{Hrvoje Benko} is a Director of Research Science at Meta Reality Labs Research where he leads a multi-disciplinary group that includes scientists and engineers with expertise in human-computer interaction, computer vision, machine learning, AI, design, neuroscience, and cognitive psychology. He has published more than 80 papers in top conferences and has received 13 best paper awards or honorable mentions, UIST Lasting Impact Award, and SIGCHI Academy Award. His website is \url{http://www.hbenko.com/}.


% \subsubsection{Pre-Workshop Engagement}
% Before the workshop, the organizers will cultivate and propose an initial set of themes to be discussed during the workshop, drawing from our prior research experiences as well as materials provided by the accepted workshop attendees. We will host a set of brief virtual sessions (with repeated sessions held in different time zones, according to participant location), where we will present our preliminary workshop plans and topics of discussion, probe participants’ enthusiasm for the proposed themes, and solicit additional interesting discussion points. The online workshops will also serve as an opportunity to start some community building before the conference workshop.
% Participants will then each deliver a 3-minute lightning talk highlighting their related research experience and 2-3 existing or potential examples of adaptive XR developments.

% % \subsection{Main Workshop Activities}


% \noindent
% \textbf{Yi Fei Cheng} is a PhD student in the Human-Computer Interaction Institute at Carnegie Mellon University, where he is advised by David Lindlbauer at the Augmented Perception Lab. His primary research interests lie in building computational models, systems, and toolkits to enable more context-aware and adaptive XR experiences. 



% \subsubsection{Provocations}
% Three externally invited experts will deliver presentations with the objective provoking further discussions. Each presentation will be followed by audience questions, moderated by the organizers. Experts will be invited to provide diverse perspectives, covering backgrounds of computational interaction, XR, and design.

% \subsubsection{Defining Future Challenges and Research Directions}
% In this final discussion session, we will begin by regrouping and refining the list of discussion topics based on the results of the first two sessions. Participants will then return to rotating between tables, but focus on discussing key challenges, opportunities, and open research questions relating to each topic.

